Tracking without bells and whistles

The problem of tracking multiple objects in a video sequence poses several challenging tasks. For tracking-by-detection, these include object re-identification, motion prediction and dealing with occlusions. We present a tracker (without bells and whistles) that accomplishes tracking without specifically targeting any of these tasks, in particular, we perform no training or optimization on tracking data. To this end, we exploit the bounding box regression of an object detector to predict the position of an object in the next frame, thereby converting a detector into a Tracktor. We demonstrate the potential of Tracktor and provide a new state-of-the-art on three multi-object tracking benchmarks by extending it with a straightforward re-identification and camera motion compensation. We then perform an analysis on the performance and failure cases of several state-of-the-art tracking methods in comparison to our Tracktor. Surprisingly, none of the dedicated tracking methods are considerably better in dealing with complex tracking scenarios, namely, small and occluded objects or missing detections. However, our approach tackles most of the easy tracking scenarios. Therefore, we motivate our approach as a new tracking paradigm and point out promising future research directions. Overall, Tracktor yields superior tracking performance than any current tracking method and our analysis exposes remaining and unsolved tracking challenges to inspire future research directions.

==> figures/teaser.tex <==
%!TEX root = ../1404.tex

\begin{figure}%[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/teaser.pdf}
    \caption{
    We present a new online multi-object tracking method without bells and whistles which pushes tracking-by-detection to the limit.
    %
    This is achieved by exploiting the object detector's bounding box regression to correct a tracked bounding box ${\bf b}^k_{t-1}$ of frame $t-1$ to the object's new position at frame $t$.
    %
    The simplicity and success of our tracker sheds reasonable doubt on more elaborate tracking methods and their shortcomings which we will discuss in a subsequent tracking-by-detection analysis on the MOT challenge~\cite{lealarxiv2015}.}
    \label{fig:teaser}
\end{figure}
